Incremental Learning in Semantic Segmentation from Image Labels

Although existing semantic segmentation approaches achieve impressive results, they still struggle to update their models incrementally as new categories are uncovered. Furthermore, pixel-by-pixel annotations are expensive and time-consuming. This paper proposes a novel framework for Weakly Incremental Learning for Semantic Segmentation, that aims at learning to segment new classes from cheap and largely available image-level labels. As opposed to existing approaches, that need to generate pseudo-labels offline, we use an auxiliary classifier, trained with image-level labels and regularized by the segmentation model, to obtain pseudo-supervision online and update the model incrementally. We cope with the inherent noise in the process by using soft-labels generated by the auxiliary classifier. We demonstrate the effectiveness of our approach on the Pascal VOC and COCO datasets, outperforming offline weakly-supervised methods and obtaining results comparable with incremental learning methods with full supervision. Code can be found at https://github.com/fcdl94/WILSON.

==> tables/pseudo-code.tex <==
\begin{algorithm}[]
\SetAlgoLined
\SetKwBlock{Localizer}{Train the \textit{localizer} $g$}{end}
\SetKwBlock{Segmentation}{Train the segmentation model $f_\theta^{t}$}{end}

\textbf{Initialize:} 
    \\Model $f_\theta^{t-1}$ pre-trained on a densely-annotated dataset with label set $\mathcal{C}^{t-1}$\;
    Model $f_\theta^{t}$ with segmentation encoder $e$\;
    \textit{Localizer} $g$\;
\textbf{Input:} 
    $\mathcal{X}$, composed by set of pixels $\mathcal{I}$ with constant cardinality $N$, with image-level annotations $y$ for novel classes $\mathcal{C}^t$\;
\textbf{Output:}
    $y=\{\text{argmax}_{c\in \mathcal{Y}^t} p_i^c\}^N_{i=1}$, $p_i^c$ the model prediction of pixel $i$ for class $c$ and $\mathcal{Y}^t$ the set of seen classes\;
 
\While{epoch in max\_epochs}{
    \For{(x,y) in $\mathcal{X}$}{
        \Localizer{
            Compute score for all classes, as $z=g(e(x))$\;
            Compute output from previous model, as $\omega = \sigma(f_\theta^{t-1}(x))$, with $\sigma(\cdot)$ as the sigmoid function\;
            Aggregate pixel-level classification scores $z$ in $\hat{y}$ as the sum of \textit{normalized Global Weighted Pooling} (Eq. 1) and \textit{focal penalty} (Eq. 2)\;
            Train $g$ on $\mathcal{C}^t$ with multi-label soft-margin loss $l_{CLS}(\hat{y}, y)$ (Eq. 3)\; 
            Train $g$ with localization prior loss $l_{LOC}(z, \omega)$ (Eq. 4)\;
            \If{$epoch \ge 5$}{
                Train $g$ with self-supervised loss $l_{SSS}$ (Eq. A3)\;
            }
        }
        Train $e$ with encoder feature distillation loss $l_{ENC}$ (Eq. A4)\;
        \If{$epoch \ge 5$}{
            \Segmentation{
                Compute hard pseudo-labels $q_i^{\text{Hard,c}}$ from $g$ (Eq. 5)\; 
                Smooth $q_i^{\text{Hard,c}}$ in $q^c$ (Eq. 6)\;
                Compute pixel-level supervision label $\hat{q}$ from $q^c$ and $f_\theta^{t-1}(x)$ (Eq. 7)\;
                Train $f_\theta$ with multi-label soft-margin loss $l_{SEG}(f_\theta^{t}(x), \hat{q})$ (Eq. 8)\;
            }
        }
    }
}
\caption{Training WILSON}
\label{pc:pseudo_code}
\end{algorithm}
